Simultaneous multi-wavelength observations of the repeating fast radio burst FRB 20190520B with Swift and FAST

Among several dozen known repeating Fast radio bursts (FRBs), those precisely localized offer the best opportunities to explore their multi-wavelength counterparts, which are key to uncovering their origins. Here we report our X-ray, ultraviolet (UV), and optical observations with the $Swift$ satellite of the repeating FRB 20190520B, in coordination with simultaneous radio observations with the Five-hundred-meter Aperture Spherical radio Telescope (FAST). Our aim was to detect potentially associated multi-wavelength bursts and identify any persistent multi-wavelength counterpart to the associated persistent radio source (PRS). While a total of 10 radio bursts were detected by FAST during the $Swift$ observations, we detected no X-ray, UV, or optical bursts in accompany with the radio bursts. We obtained the energy upper limits ($3\sigma$) on any multi-wavelength bursts as follows: $5.03 \times 10^{47}$ erg in the hard X-ray band (15--150 keV), $7.98 \times 10^{45}$ erg in the soft X-ray band (0.3--10 keV), and $4.51 \times 10^{44}$ erg in the U band (3465\AA), respectively. The energy ratio between soft X-ray (0.3--10 keV) and radio emission of the bursts is constrained as $<6\times10^{7}$, and the ratio between optical (U band) and radio as $<1.19\times10^{6}$. We detect no multi-wavelength counterpart to the PRS. The 3$\sigma$ luminosity upper limits are 1.04$\times10^{47}$ (15--150 keV), 8.81$\times10^{42}$ (0.3--10 keV), 9.26$\times10^{42}$ (UVW1), and 2.54$\times10^{42}$ erg s$^{-1}$ (U), respectively. We show that the PRS is much more radio loud than representative pulsar wind nebulae, supernova remnants, extended jets of Galactic X-ray binaries, and ultraluminous X-ray sources, suggestive of boosted radio emission of the PRS.

==> old_table_fig.tex <==
\begin{table*}
\centering
%\scriptsize
\caption{Burst upper limit from XRT on time scale of 2.51s. }
\label{tab:xrt_burst}

\begin{tabular}{cccccc}
\hline

burst time$^{a}$ & XRT time     &    Count Rate $^{b}$  & Luminosity & Energy & $E_{\rm X}/E_{\rm R}$ $^{c}$\\
 (MJD)     &  (MJD)                      &     (c/s) & ($10^{46}$ erg s$^{-1}$) & ($10^{46}$ erg)  & $\times10^{8}$\\
\hline 
58991.728910176&58991.728923501&$<$3.58&$<$3.66&$<$9.19&$<$5.47 \\
59067.484320871&59067.484320859&$<$3.45&$<$3.53&$<$8.87&$<$5.58 \\
59067.484321450&59067.484320859&$<$3.45&$<$3.53&$<$8.87&$<$4.98  \\
59071.470478456&59071.470485296&$<$3.63&$<$3.72&$<$9.34&$<$9.73 \\
59071.470478688&59071.470485296&$<$3.63&$<$3.72&$<$9.34&$<$11.54  \\
59075.452687489&59075.452698807&$<$3.20&$<$3.28&$<$8.22&$<$2.16 \\
59075.453197005&59075.453192673&$<$3.20&$<$3.28&$<$8.23&$<$3.23 \\
59077.496337171&59077.496344162&$<$3.53&$<$3.62&$<$9.08&$<$5.41  \\
59077.496488380&59077.496489417&$<$3.54&$<$3.63&$<$9.10&$<$8.35  \\
59077.497491638&59077.497477148&$<$3.54&$<$3.62&$<$9.10&$<$7.98  \\
 \hline 
\end{tabular}   

\footnotesize
\begin{itemize}
\item [$^a$] The burst time is at Coordinated Universal Time (UTC), which is referenced to infinite frequency.
\item [$^b$] This is $3\sigma$ upper limit.
\item [$^c$] The ratio between X-ray and radio energy. 
    
\end{itemize}
\end{table*}



\begin{table*}
\centering
%\scriptsize
\caption{Burst upper limit in the $U$-band on time scale of 12 ms}
\label{tab:uvot_burst}
\begin{tabular}{cccccc}
\hline

burst time$^{a}$ & U time    &  AB Mag$^{b}$  & Luminosity   & Energy & $E_{\rm U}/E_{\rm R}$ $^{c}$\\
   (MJD)   &  (MJD)           &     &  ($10^{46}$ erg s$^{-1}$) & ($10^{44}$ erg)       &  $\times10^{6}$   \\
\hline
59067.484320871&59067.484320927&$<$12.93&$<$3.76&$<$4.51&$<$2.83  \\
59067.484321450&59067.484321482&$<$12.93&$<$3.76&$<$4.51&$<$2.53  \\
59071.470478456&59071.470478477&$<$12.93&$<$3.76&$<$4.51&$<$4.70 \\
59071.470478688&59071.470478755&$<$12.93&$<$3.76&$<$4.51&$<$5.56 \\
59075.452687489&59075.452687499&$<$12.93&$<$3.76&$<$4.51&$<$1.19  \\
59075.453197005&59075.453196944&$<$12.93&$<$3.76&$<$4.51&$<$1.77 \\
59077.496337171&59077.496337235&$<$12.93&$<$3.76&$<$4.51&$<$2.68 \\
59077.496488380&59077.496488346&$<$12.93&$<$3.76&$<$4.51&$<$4.14 \\
59077.497491638&59077.497491680&$<$12.93&$<$3.76&$<$4.51&$<$3.95 \\
\hline 
\end{tabular}   

\footnotesize
\begin{itemize}
\item [$^a$] The burst time is at Coordinated Universal Time (UTC), which is referenced to infinite frequency.
\item [$^b$] This is $3\sigma$ upper/lower limit. The time resolution of the $U$-band is 12 ms.
\item [$^c$] The ratio between U-band and radio energy. 
\end{itemize}

\end{table*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{XRT_sum_img.pdf}
    \caption{The stacked image of all the XRT observations. The green cross marks the \FRB position. The upper right bright point source is a bright star V* V1042 Sco.}
    \label{fig:XRT}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{all_U_sum_center.pdf}
    \caption{The stacked image in the $U$-band of UVOT. The green cross marks the \FRB position. The upper right brightest star corresponds to the nearby X-ray point source seen with XRT. }
    \label{fig:U}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{BAT_survey_img.pdf}
    \caption{The $Swift$/BAT hard X-ray survey image obtained from obsID 00013503003. The bright persistent source is Sco~X-1. The greens cross markes the VLA position of \FRB.
    }
    \label{fig:bat_image}
\end{figure}


\begin{table*}%
\caption{ The properties of the ? FRB bursts covered by $Swift$ observations.
\label{tab:bursttab}}
\scriptsize
\begin{tabular}  {cc c c c  c c}
\hline%
\hline%
%Burst\ ID & Burst time & DM & Pulse Width & Bandwidth & Scatter tail & Fluence & Energy\\%
Burst  ID & Burst time & DM &  Bandwidth  & Energy  \\
%          & (MJD)      & ($\dmu$)   & (ms) & (GHz)  & (mJy/ms) & ($\times10^{37}$erg) \\
\hline%
%7 & 58991.684351079 & 1200.4(20.8) & 17.5(2.0) & 1300-1450 & 0.0(0.0) & 0.0(0.0
%) \\
%8 & 58991.686137870 & 1200.4(20.8) & 9.9(1.2) & 1360-1450 & 0.0(0.0) & 0.0(0.0
%) \\
%9 & 58991.686875951 & 1200.4(20.8) & 14.7(1.5) & 1300-1450 & 0.0(0.0) & 0.0(0.0
%) \\
%10 & 58991.704636888 & 1200.4(20.8) & 18.5(1.6) & 1350-1450 & 0.0(0.0) & 0.0(0.0
%) \\
%11 & 58991.704638485 & 1200.4(20.8) & 20.7(1.2) & 1370-1450 & 0.0(0.0) & 0.0(0.0
%) \\
%12 & 58991.717697335 & 1200.4(20.8) & 11.8(0.7) & 1300-1450 & 0.0(0.0) & 0.0(0.0
%) \\
%13 & 58991.717878516 & 1200.4(20.8) & 14.9(2.7) & 1200-1450 & 0.0(0.0) & 0.0(0.0
%) \\
%14 & 58991.718217265 & 1200.4(20.8) & 17.9(1.4) & 1360-1450 & 0.0(0.0) & 0.0(0.0
%) \\
%15 & 58991.718217670 & 1200.4(20.8) & 16.8(1.1) & 1360-1450 & 0.0(0.0) & 0.0(0.0
%) \\
16 & 58991.718218082 & 1200.4(20.8) & 19.1(1.1) & 1270-1450 & 0.0(0.0) & 0.0(0.0
) \\
%17 & 58991.735450006 & 1200.4(20.8) & 20.9(1.7) & 1300-1450 & 0.0(0.0) & 0.0(0.0
%) \\
%18 & 58991.750640038 & 1200.4(20.8) & 25.1(5.8) & 1300-1450 & 0.0(0.0) & 0.0(0.0
%) \\
%19 & 58991.750640790 & 1200.4(20.8) & 25.5(4.3) & 1200-1450 & 0.0(0.0) & 0.0(0.0
%) \\
35 & 59067.467544345 & 1201.9(21.0) & 7.4(1.0) & 1200-1400 & 0.0(0.0) & 0.0(0.0
) \\
36 & 59067.486738799 & 1201.9(21.0) & 16.9(2.0) & 1300-1450 & 0.0(0.0) & 0.0(0.0
) \\
37 & 59067.486739378 & 1201.9(21.0) & 18.2(2.0) & 1050-1300 & 0.0(0.0) & 0.0(0.0
) \\
38 & 59067.502691880 & 1201.9(21.0) & 20.3(6.5) & 1120-1220 & 0.0(0.0) & 0.0(0.0
) \\
39 & 59067.509899127 & 1201.9(21.0) & 13.3(1.7) & 1250-1400 & 0.0(0.0) & 0.0(0.0
) \\
40 & 59067.535246460 & 1201.9(21.0) & 8.4(1.0) & 1300-1450 & 0.0(0.0) & 0.0(0.0
) \\
41 & 59069.495909561 & 1201.9(21.0) & 14.3(2.0) & 1270-1450 & 0.0(0.0) & 0.0(0.0
) \\
42 & 59069.501196109 & 1201.9(21.0) & 22.3(1.4) & 1300-1450 & 0.0(0.0) & 0.0(0.0
) \\
43 & 59069.514994796 & 1201.9(21.0) & 12.9(1.1) & 1300-1450 & 0.0(0.0) & 0.0(0.0
) \\
44 & 59071.472522775 & 1201.9(21.0) & 2.0(0.6) & 1340-1450 & 0.0(0.0) & 0.0(0.0
) \\
45 & 59071.472523007 & 1201.9(21.0) & 6.0(0.8) & 1340-1450 & 0.0(0.0) & 0.0(0.0
) \\
46 & 59071.491696655 & 1201.9(21.0) & 11.2(1.8) & 1300-1450 & 0.0(0.0) & 0.0(0.0
) \\
47 & 59073.496887082 & 1200.0(16.0) & 10.7(2.3) & 1250-1450 & 0.0(0.0) & 0.0(0.0
) \\
48 & 59073.515256071 & 1200.0(16.0) & 6.8(0.7) & 1350-1450 & 0.0(0.0) & 0.0(0.0
) \\
49 & 59073.515256881 & 1200.0(16.0) & 16.1(6.3) & 1160-1360 & 0.0(0.0) & 0.0(0.0
) \\
50 & 59075.454353002 & 1200.0(16.0) & 32.1(2.2) & 1050-1180 & 0.0(0.0) & 0.0(0.0
) \\
51 & 59075.454862469 & 1200.0(16.0) & 32.4(2.5) & 1250-1450 & 0.0(0.0) & 0.0(0.0
) \\
52 & 59075.472181012 & 1200.0(16.0) & 11.6(1.8) & 1260-1400 & 0.0(0.0) & 0.0(0.0
) \\
53 & 59075.484186304 & 1200.0(16.0) & 9.9(1.0) & 1100-1400 & 0.0(0.0) & 0.0(0.0
) \\
54 & 59075.496463775 & 1200.0(16.0) & 17.2(2.7) & 1150-1450 & 0.0(0.0) & 0.0(0.0
) \\
55 & 59077.448938437 & 1200.0(16.0) & 8.0(1.2) & 1200-1400 & 0.0(0.0) & 0.0(0.0
) \\
56 & 59077.448939131 & 1200.0(16.0) & 8.0(1.4) & 1250-1450 & 0.0(0.0) & 0.0(0.0
) \\
57 & 59077.449538432 & 1200.0(16.0) & 16.1(1.4) & 1280-1400 & 0.0(0.0) & 0.0(0.0
) \\
58 & 59077.449939184 & 1200.0(16.0) & 49.9(6.4) & 1280-1450 & 0.0(0.0) & 0.0(0.0
) \\
59 & 59077.449939372 & 1200.0(16.0) & 32.6(3.5) & 1050-1450 & 0.0(0.0) & 0.0(0.0
) \\
60 & 59077.460100338 & 1200.0(16.0) & 8.0(0.9) & 1300-1450 & 0.0(0.0) & 0.0(0.0
) \\
61 & 59077.460503968 & 1200.0(16.0) & 10.0(1.2) & 1250-1450 & 0.0(0.0) & 0.0(0.0
) \\
62 & 59077.466295203 & 1200.0(16.0) & 10.5(1.0) & 1250-1400 & 0.0(0.0) & 0.0(0.0
) \\
63 & 59077.468715062 & 1200.0(16.0) & 18.6(2.2) & 1050-1250 & 0.0(0.0) & 0.0(0.0
) \\
64 & 59077.469903193 & 1200.0(16.0) & 13.9(1.5) & 1250-1450 & 0.0(0.0) & 0.0(0.0
) \\
65 & 59077.475047947 & 1200.0(16.0) & 11.6(1.3) & 1200-1450 & 0.0(0.0) & 0.0(0.0
) \\
66 & 59077.475330491 & 1200.0(16.0) & 17.9(0.9) & 1250-1450 & 0.0(0.0) & 0.0(0.0
) \\
67 & 59077.477447949 & 1200.0(16.0) & 5.2(3.0) & 1300-1450 & 0.0(0.0) & 0.0(0.0
) \\
68 & 59077.485451841 & 1200.0(16.0) & 19.9(1.4) & 1340-1450 & 0.0(0.0) & 0.0(0.0
) \\
69 & 59077.485451957 & 1200.0(16.0) & 15.8(0.9) & 1270-1450 & 0.0(0.0) & 0.0(0.0
) \\
70 & 59077.490027004 & 1200.0(16.0) & 5.3(0.7) & 1350-1450 & 0.0(0.0) & 0.0(0.0
) \\
71 & 59077.491413589 & 1200.0(16.0) & 11.9(2.0) & 1300-1450 & 0.0(0.0) & 0.0(0.0
) \\
72 & 59077.497806611 & 1200.0(16.0) & 13.8(1.4) & 1200-1450 & 0.0(0.0) & 0.0(0.0
) \\
73 & 59077.497957805 & 1200.0(16.0) & 8.5(0.8) & 1200-1450 & 0.0(0.0) & 0.0(0.0
) \\
74 & 59077.498960966 & 1200.0(16.0) & 7.2(0.9) & 1200-1450 & 0.0(0.0) & 0.0(0.0
) \\

\hline
\end{tabular}  
\end{table*}

